Exact analytical solutions in inhomogeneous magnetic fields for linear asteroseismic waves

We solve for waves in an isothermal, stratified medium with a magnetic field that points along a direction perpendicular to that of gravity and varies exponentially in the direction of gravity. We find exact analytical solutions for two different cases: (a) waves propagating along the direction of the magnetic field and (b) waves propagating along the direction of the gravity. In each case, we find solutions in terms of either the hypergeometric functions or their confluent cousins. We solve the resultant transcendental dispersion relation numerically. The changes in the eigenfrequencies due to a spatially inhomogeneous Alfv\'en wave speed are significant -- there are more oscillations or leaking of nodes of the eigenfunctions in regions of lower Alfv\'en speed and wave reflection from regions of larger Alfv\'en speed. Such changes in the dispersion relation and the mode structures may allow detection of magnetic fields buried in the stellar interior.

==> rmv.tex <==
found magnetohydrostatic equilibrium
       solution for an arbitrarily varying non-uniform magnetic field, and

% physics (see, e.g., the review by \citealt{christ2002}). So is the hope with the
% emerging asteroseismology, which allows to extract sub-surface structures and
% properties of the stars with reliable accuracy~ \citep{hekker2017, aerts2019}.

% In stars including Sun-like, however, stronger magnetic fields generally brew deep within the star and the waves near the stellar surface might be affected in a manner different from the theoretical consideration where the uniform magnetic fields permeate throughout the space. The latter although useful is an idealization; the former, however, is a bit closer to the realistic circumstances. It is not fully clear whether the former is different from the latter and if so, how. The goal of this article is to clarify this. Being an inverse problem, it is also likely to shed light on constraining magnetic fields in the stellar interior, based on the observed frequencies of stellar oscillations \citep{fuller2015asteroseismology}. Since analytical progress is favored here, the system with \textit{inhomogeneous magnetic fields} will be explored with as much generality as possible, while relaxing other complications if needed.


% The analytical solution for the non-trivial magnetic field configuration has usefulness also, apart from examining the effect on linear eigenfrequencies, in advancing nonlinear asteroseismology. The nonlinear oscillations are commonly and convienently analysed in a weakly nonlinear framework where a constraint of resonant interactions is considered (i.e., the assumption of frequency mismatch of three waves being almost close to zero). This is certainly helpful to begin making progress in the nonlinear asteroseismology \citep{weinberg2019, weinberg2021}. To go beyond, here, we shall relax the latter constraint of resonant three-wave coupling, and illustrate a general framework of three-wave mode coupling analysis where the exact solutions of linear waves can be employed in service. We conjecture that these nonlinear interactions are subject to modulations as the stellar magnetic fields in the stellar interior brew due to dynamo activity and can cause the deep buried signals of seismic waves to be transmitted towards the stellar surface. More quantitative work, however, is needed for such an understanding. Here, we shall be satisfied with a step towards this.

% \underline{Old text:} {\color{red} For a constant magnetic field acting
% in the $x$ direction, with a background density that varies
% exponentially as a function of the vertical coordinate, this problem
% was solved  for waves propagating along the direction of the magnetic field (the $x$
% direction) by \cite{nye1976, adam1977occurrence},\cite[see also,][for a more comprehensive treatment]{thomas1983magneto} and for waves propagating along the
% direction of gravity (the $z$ direction)  by
% \cite{campos1983three}. In both of these cases, it is possible to find
% an exact solution that uses the hypergeometric functions.
% \cite{campos2015combined} generalized the latter to the one where
% the magnetic field is also an exponential function of the vertical
% coordinate $z$, with a characteristic length scale $\lB$,
% but its direction remains fixed -- along the $x$ direction.
% For the particular case where $\lB$ is twice the density scale height,
% $\lrho$, \cite{campos2015combined} found an exact solution for waves propagating along the gravity field in terms of
% confluent hypergeometric functions. The problem remains unsolved for
% any value of $\lB/\lrho$, not equal to two as well as for waves
% propagating along the $x$ direction -- the direction of the magnetic
% field and along the $y$ direction -- the direction
% orthogonal to both the direction of the magnetic field and the
% direction of gravity. } 




% For simplicity, one can consider a Cartesian slab of plasma with constant gravity acting in the
% negative $z$ direction as shown in \fig{fig:sketch}. Assume the temperature to be a constant.
% Furthermore, assume periodic boundary conditions in the horizontal $(x,y)$ directions. In the absence of magnetic field, a static solution
% of the equations of magnetohydrodynamics (MHD) is realizable; the density $\rho =\rhon(z)$ is a function of the vertical coordinate $z$ alone and the velocity is zero everywhere. It is straightforward to apply the theory of linear waves to this problem.  Due to the symmetry of the problem, the dynamical variables -- velocity or Lagrangian displacement and density -- can be written down as $\exp i(k_x x + k_y y - \omega t)$, multiplied by a function of the vertical coordinate $z$. In particular, the $z$ component of the Lagrangian displacement satisfies a second order differential equation in $z$, \cite[see, e.g., ][section 4]{tolstoy1963theory}. By solving this equation with proper boundary conditions, we can find out the dispersion relation of the waves in this setup. How would this dispersion relation change in the presence of a horizontal magnetic field? For a constant magnetic field acting in the $x$ direction, with a background density that varies exponentially as a function of the vertical coordinate, this problem was solved  for waves propagating along the direction of the magnetic field (the $x$ direction) by \cite{nye1976solar, adam1977occurrence},\cite[see also,][for a more comprehensive treatment]{thomas1983magneto} and for waves propagating along the direction of gravity (the $z$ direction)  by \cite{campos1983three}. In both of these cases, it is possible to find an exact solution that uses the hypergeometric functions. \cite{campos2015combined} generalized the latter to the one where the magnetic field is also an exponential function of the vertical coordinate $z$, with a characteristic length scale $\lB$, but its direction remains fixed -- along the $x$ direction. For the particular case where $\lB$ is twice the density scale height, $\lrho$, \cite{campos2015combined} found an exact solution for waves propagating along the gravity field in terms of confluent hypergeometric functions. The problem remains unsolved for any value of $\lB/\lrho$, not equal to two as well as for waves propagating along the $x$ direction -- the direction of the magnetic field and along the $y$ direction -- the direction orthogonal to both the direction of the magnetic field and the direction of gravity.

%In this work, we also illustrate how such linear wave solution can be utilized to compute the nonlinear mode coupling coefficients, which is a central part of emerging nonlinear asteroseismology.

%-------------------------
\begin{widetext}
\begin{equation}
M
=
\begin{bmatrix}
    \begin{array}{c|c|c}
        \omega^2-{k_x}^2 & -k_x k_y & {-i k_x/ \gmad}  \\ \hline
        -k_x k_y & \omega^2 - {k_y}^2 - k^2  \frac{{B_0}^2}{\rho_0\MaA^2}  & {-i k_y/ \gmad}  \\ \hline
        i k_x \left({\frac{1}{\gmad}-1}-\frac{\gmad}{2\MaA^2}\frac{D{(B_0)}^2}{\rho_0} \right) & i k_y \left({\frac{1}{\gmad}-1}+ \frac{2-\gmad}{2\MaA^2}\frac{D{(B_0)}^2}{\rho_0} \right)  & \omega^2  - \frac{{B_0}^2}{\rho_0\MaA^2}k_x^2
    \end{array}
\end{bmatrix}
\end{equation}
\end{widetext}
and 
\begin{equation}
N
=
\begin{bmatrix}
    \begin{array}{c|c|c}
        0 & 0 & i k_x  \\ \hline
        0 & 0 & i k_y \left(1 + \frac{{B_0}^2}{\rho_0\MaA^2} \right) \\ \hline
        i k_x & i k_y \left(1 + \frac{{B_0}^2}{\rho_0\MaA^2} \right)  & \frac{2-\gmad}{2\MaA^2} \frac{D{(B_0)}^2}{\rho_0} {- 1}
    \end{array}
\end{bmatrix}.
\end{equation}


% This relation is valid as long as,
% \begin{equation}
%     \left| -\frac{B_2(\omega,k)}{A_2(\omega,k)} \right| < 1,
% \end{equation}
% holds true. When not true, other representation of the hypergeometric function is needed.





% \section{Further application: linear modes in nonlinear coupling coefficient} \label{sec:applicationNL}
% Here we transform the nonlinear MHD equations from the physical space to the eigenmode space (which is a mere change of basis) to compute the nonlinear coupling coefficient of the linear eigenmodes of stellar oscillations. This new branch of asteroseismology as-of-yet is still in its infancy and very little, apart from speculations, is known about the imprints of nonlinear mode interactions on the observed oscillations. Below we illustrate how linear eigenmodes, found either numerically or derived analytically like in this article, can be employed to evaluate the nonlinear mode coupling strengths.

% Since the method about to be presented is generic and is likely to help advance emerging nonlinear asteroseismology, we consider, in this section, completely arbitrary background profiles. Consider an arbitrary perturbation, $X = \left[\widetilde{\rho}, \widetilde{\mathbf{u}}, \widetilde{\mathbf{b}}, \widetilde{p}  \right]$. The nonlinear MHD equations, up to quadratic nonlinear terms\footnote{Higher-order nonlinearities also exist, however they are conventionally and conveniently assumed to be of lesser significance. For the problem at hand of the stellar oscillations, quadratic nonlinearity can be already quite sufficient as the frequencies of the observed oscillations are very close to the linear eigenfrequencies, but with somewhat broadband spectrum possibly due to the turbulence generating the waves.}, assume its general form,
% \begin{equation} \label{eq:nonlinphys}
%     \partial_t X = \mathcal{L} X + \mathcal{N}(X,X),
% \end{equation}
% where the linear operator depends on the background fields, $\rho_0, \mathbf{U}_0, \mathbf{B}_0, p_0$. Here, we consider $\mathbf{U}_0=0$. Fourier transforming the above equation along the $x$- and $y$-directions,
% \begin{equation}
% \begin{aligned}
%     \partial_t X(k_x, k_y) = \mathcal{L} &X(k_x, k_y)\\
%     &+ \sum_{k_x^{'}, k_y^{'}}\mathcal{N}\left[X(k_x^{'}, k_y^{'}),X(k_x^{''}, k_y^{''})\right],
% \end{aligned}
% \end{equation}
% where the familiar selection rules, $k_x^{''}+k_x^{'}=k_x$ and $k_y^{''}+k_y^{'}=k_y$, arise from the orthogonality of the Fourier modes and hence are to be imposed. Henceforth, for brevity, we shall write $X(k_x^{'}, k_y^{'})$ as $X^{'}$ and $X(k_x^{''}, k_y^{''})$ as $X^{''}$. The perturbation $X(k_x, k_y)$ will be written simply as $X$ unless a need arises to distinguish it. Until now, the $x$- and $y$-coordinates have been transformed to the Fourier wavenumbers $k_x$ and $k_y$, respectively. We shall now transform the inhomogeneous direction, $z$-coordinate to the eigenmodes, which are not Fourier ones, but can be hypergeometric functions or some unnamed purely numerical eigenmodes if numerical eigenvalue solver is being employed to find the eigenmodes. Such eigenmodes will be counted with the index $r$ and denoted by $X_r(k_x, k_y, z)$. Note each eigenmode has a particular structure in the $z$-axis. Since the linear operator at hand is Hermitian, its eigenmodes are guaranteed to form a complete basis and thus an arbitrary perturbation can be expanded on this basis as $X(x,y,z,t) = \sum_{k_x, k_y} \left[X(k_x, k_y, z, t)\right] e^{i (k_x x+ k_y y)} = \sum_{k_x, k_y} \left[ \sum_r \beta_r(k_x, k_y, t) X_r(k_x, k_y, z)\right] e^{i (k_x x+ k_y y)}$. Progress is made now by rewriting the nonlinear MHD equations on this eigenmode basis,
% \begin{widetext}
% \begin{equation} \label{eq:betatimederv}
%     \sum_r \partial_t \beta_r(k_x, k_y) X_{r, k_x, k_y} 
%     =\sum_r \beta_r(k_x, k_y)
%     \mathcal{L} X_{r, k_x, k_y}
%     + \sum_{k_x^{'}, k_y^{'}} \sum_{p,q} \beta_p^{'} \beta_q^{''} \mathcal{N}(X_p^{'}, X_q^{''}),
% \end{equation}
% where the linear operator $\mathcal{L}$ is,
% \scriptsize
% \begin{equation}\begin{bmatrix}
%     \begin{array}{c c c c c c c c}
%         0 & -\rho_0 i k_x & -\rho_0 i k_y & \partial_z \rho_0 -\rho_0 \partial_z & 0 & 0 & 0 & 0 \\
%         0 & 0 & 0 & 0 & \overline{B}_y ik_y +\overline{B}_z \partial_z  & -\overline{B}_y ik_x  & \partial_z \overline{B}_x -\overline{B}_z ik_x & ik_x/\rho_0 \\
%         0 & 0 & 0 & 0 & -\overline{B}_x ik_y & \overline{B}_y ik_x + \overline{B}_z \partial_z & -\overline{B}_z ik_y + \partial_z \overline{B}_y & -ik_y/\rho_0 \\
%         -g/\rho_0 & 0 & 0 & 0 & -\overline{B}_x \partial_z -\partial_z \overline{B}_x & -\overline{B}_y \partial_z -\partial_z \overline{B}_y & \overline{B}_x ik_x+\overline{B}_y ik_y & -\partial_z /\rho_0 \\
%         0 & B_x ik_x+B_y ik_y + B_z \partial_z & 0 & -\partial_z B_x & 0 & 0 & 0 & 0 \\
%         0 & 0 & B_x ik_x+B_y ik_y + B_z & -\partial_z B_y & 0 & 0 & 0 & 0 \\
%         0 & 0 & 0 & B_x ik_x+B_y ik_y + B_z & 0 & 0 & 0 & 0 \\
%         0 & -ik_x c_s^2 \rho_0 & -ik_y c_s^2 \rho_0 & -\partial_z (\rho_0 c_s^2)/\gamma -\rho_0 c_s^2 \partial_z & 0 & 0 & 0 & 0 \\
%     \end{array}
%     \end{bmatrix},
% \end{equation}
% \normalsize
% with $\overline{B}_{j} = B_{j}/(\mu_0 \rho_0)$ and the nonlinear operator $\mathcal{N}(X_p^{'}, X_q^{''})$, using Einstein summation notation, is written as,
% \begin{equation}
%     \begin{bmatrix}
%     \begin{array}{c}
%         \mathcal{N}_1\\
%         \mathcal{N}_2\\
%         \mathcal{N}_3\\
%         \mathcal{N}_4\\
%         \mathcal{N}_5\\
%         \mathcal{N}_6\\
%         \mathcal{N}_7\\
%         \mathcal{N}_8\\
%     \end{array}
%     \end{bmatrix}_{p,q}
%     =
%     \begin{bmatrix}
%     \begin{array}{c}
%         -\tilde{u}_\gamma^{'} \partial_\gamma \tilde{\rho}^{''} -\tilde{\rho}^{'} \partial_\gamma \tilde{u}_\gamma^{''}\\
%         \mathcal{Q}(\alpha=x)\\
%         \mathcal{Q}(\alpha=y)\\
%         \mathcal{Q}(\alpha=z)\\
%         \tilde{b}_\gamma^{'} \partial_\gamma  \tilde{u}_x^{''}-\tilde{u}_\gamma^{'} \partial_\gamma \tilde{b}_x^{''}\\
%         \tilde{b}_\gamma^{'} \partial_\gamma  \tilde{u}_y^{''}-\tilde{u}_\gamma^{'} \partial_\gamma \tilde{b}_y^{''}\\
%         \tilde{b}_\gamma^{'} \partial_\gamma  \tilde{u}_z^{''}-\tilde{u}_\gamma^{'} \partial_\gamma \tilde{b}_z^{''}\\
%         -\tilde{u}_\gamma^{'} \partial_\gamma \tilde{p}^{''} -c_s^2 \tilde{\rho}^{'} \partial_\gamma \tilde{u}_\gamma^{''}
%     \end{array}
%     \end{bmatrix}_{p,q},
% \end{equation}
% with
% \begin{equation}
% \mathcal{Q}(\alpha) = 
%         -\tilde{u}_\beta^{'} \partial_\beta \tilde{u}_\alpha^{''} + \epsilon_{\alpha \beta \gamma} \epsilon_{\beta \delta \zeta} \frac{\tilde{b}_\gamma^{'} \partial_\delta \tilde{b}_\zeta^{''}}{\mu_0 \rho_0} - \left\{-\frac{\partial_\alpha \tilde{p}^{'}}{\rho_0} -\frac{g \delta_{\alpha 3} \tilde{\rho}}{\rho_0} + \epsilon_{\alpha \beta \gamma} \epsilon_{\beta \delta \zeta} \frac{B_\gamma \partial_\delta \tilde{b}_\zeta^{'}}{\mu_0 \rho_0} + \epsilon_{\alpha \beta \gamma} \epsilon_{\beta \delta \zeta} \frac{ \partial_\delta \tilde{B}_\zeta \tilde{b}_\gamma^{'}}{\mu_0 \rho_0} \right\} \frac{\tilde{\rho}^{''}}{\rho_0}.
% \end{equation}
% In the above equation, no assumption has been made apart from the equations are dissipationless, the mean flow is non-existent, and all the background fields vary only along the $z$-axis; however, they can point in any direction in $3$-dimensional space. The equation of state is also not yet specified; the motions above are considered isentropic as conventional. (Changes to the last assumption is not difficult to implement.)

% The above equation \eqref{eq:betatimederv} for the mode amplitude is completely equivalent to the nonlinear MHD equations in physical space, i.e., Eq.~\eqref{eq:nonlinphys}. 

% Note that Eq.~\eqref{eq:betatimederv} still has a summation over all the eigenmodes on the left-hand side. Now, to obtain the mode amplitude evolution equation for each eigenmode, e.g., a fast (pressure-dominated) mode, a slow (gravity-dominated) mode, or a shear-Alfvén mode (i.e., $p-$, or $g-$ or $a-$mode), we exploit the orthogonality of the eigenfunctions of the Hermitian operator $\mathcal{L}$, by multiplying the above equation with a row vector containing a proper weight factor, $\bf{w}(z)$, such that the eigenfunctions are orthogonal under this inner product. Thus multiplying the above equation with the properly chosen row vector, also called the left eigenvector,
% $X_{\mathrm{left}} =  \left[w_1(z)\tilde{\rho},\ \ w_2(z)\tilde{u}_x,\ \  w_3(z)\tilde{u}_y,\ \  w_4(z)\tilde{u}_z,\ \  w_5(z)\tilde{b}_x,\ \   w_6(z)\tilde{b}_y,\ \  w_7(z)\tilde{b}_z,\ \  w_8(z)\tilde{p} \right]_{l, k_x, k_y}^{\ast}$, and integrating along the $z$-axis across the domain, one arrives at the mode amplitude evolution equation of an individual eigenmode,
% \begin{equation} \label{eq:NLcouplingevoln}
% \begin{aligned}
%     \partial_t \beta_{l, k_x, k_y} &= i \omega_{l, k_x, k_y} \beta_{l, k_x, k_y} + \sum_{k_x^{'}, k_y^{'}, p, q} \beta_{p}^{'} \beta_{q}^{''} \left[\int_z dz \left\{w_1^\ast \tilde{\rho}_l^\ast \mathcal{N}_1 + w_2^\ast \tilde{u}_{x,l}^\ast \mathcal{N}_2 + \hdots + w_8^\ast \tilde{p}_l^\ast \mathcal{N}_8 \right\}\right]\\
%     &= i \omega_{l, k_x, k_y} \beta_{l, k_x, k_y} + \sum_{k_x^{'}, k_y^{'}, p, q} \beta_{p}^{'} \beta_{q}^{''} \ \ C_{p, q}^{l}(k_x, k_x^{'}, k_y, k_y^{'}, \MaA).
% \end{aligned}
% \end{equation}
% \end{widetext}
% % Note that the hypergeometric functions are orthogonal to each other with a weight factor $w(z) = z^{\alpha} (1-z)^{\beta}$ where $\alpha$ and $\beta$ are related to the arguments, $A,B, C$, of the Gauss hypergeometric functions.

% Multiplying above with the left eigenvector diagonalizes the linear operator, i.e., diagonal entries of the product are the eigenvalues $\omega_{l, k_x, k_y}$ of the linear operator. This is tantamount to solving for the dispersion relation of the linear waves. If a numerical eigenvalue solver is being requested for the numerical eigenmodes, computation of the left eigenvector is readily available by taking Hermitian conjugation of the linear operator. The diagonalization procedure is guaranteed due to the property that the left and right eigenvectors are always are orthogonal to each other (even for non-Hermitian matrices). 

% The nonlinear mode coupling coefficient between two linear eigenmodes $p$ and $q$, driving a third eigenmode $l$, all at different wavenumbers, can be written from Eq.~\eqref{eq:NLcouplingevoln} as,
% \begin{equation}
% \begin{aligned}
%   C_{p, q}^{l}(k_x, &k_x^{'}, k_y, k_y^{'}, \MaA) \\
%   &= \int_z dz \left\{w_1^\ast \tilde{\rho}_l^\ast \mathcal{N}_1^{p,q} + \hdots + w_8^\ast \tilde{p}_l^\ast \mathcal{N}_8^{p,q} \right\}.
% \end{aligned}
% \end{equation}
% In particular, one would like to study the behavior of $C_{p=-1, q=-1}^{l=+1}$ as a function of $\MaA$, that is to say, the modulation of $g+g$ interaction driving a $p-$mode\footnote{Conventional notation is used here, i.e., different $p$- and $g$-modes are denoted by $+1, +2, +3, ..$ and $-1, -2, -3, ..$, respectively.}. The impact of the presence of a magnetic field or lack thereof on this $g+g \rightarrow p$ interaction would be valuable to identify, which possibly could help put reliable constraints on the interior magnetic fields. Since the exact analytical solution for the linear eigenmodes is presented here, direct numerical integration of the product of three hypergeometric functions is available -- without having to beg an eigenvalue solver to provide us the numerical eigenmodes in the first place. The numerical integration, however, will not be performed here as it is beyond the purview of this work where we present the heretofore unknown exact solutions to the linear eigenmodes in inhomogeneous magnetic fields and outline the method to apply such solutions for making progress with generic nonlinear asteroseismology.

% As closing remarks, we note that there have been recent interests in evaluating the nonlinear coupling coefficients and learning the nonlinearity's imprints on the observed stellar oscillations \citep{weinberg2021, beeck2021, guo2020, weinberg2019, weinberg2012}. This allows better and deeper probing of the interior of stars. Such exciting and useful endeavors can benefit from benchmarking tests that are rooted on the analytical exact solutions and offer nonlinear mode coupling strengths. Calculations presented herein can thus help benchmark the numerical codes that are being developed. Asymptotic analysis of the nonlinear mode coupling coefficient, by employing the exact analytical linear eigenmodes is another possible avenue to reap qualitative understanding. Future research along these directions can help make substantial progress in the nonlinear asteroseismology and thus such investigation is merited.

